On the Expressiveness of a Logic of Separated Relations

We compare the model-theoretic expressiveness of the existential fragment of Separation Logic over unrestricted relational signatures (SLR) -- with only separating conjunction as logical connective and higher-order inductive definitions, traditionally known as the symbolic heap fragment -- with the expressiveness of (Monadic) Second Order Logic ((M)SO). While SLR and MSO are incomparable on structures of unbounded treewidth, it turns out that SLR can be embedded in SO, in general, and that MSO becomes a strict subset of SLR, when the treewidth of the models is bounded by a parameter given as input. We also discuss the problem of defining a fragment of SLR that is equivalent to MSO over models of bounded treewidth. Such a fragment would then become the most general Separation Logic with a decidable entailment problem, a key ingredient of practical verification methods for self-adapting (reconfigurable) component-based and distributed systems.

==> mso-sid.tex <==
We first build a generic SID that defines all structures $\struc$,
over a given signature $\signature$, such that $\twof{\struc} \le k$,
according to Definition~\ref{def:treewidth}.

\begin{definition}\label{def:reduced-td}
A tree decomposition $\tree=(\tnodes,\tedges,r,\alabel)$ of a
structure $\struc$ is said to be \emph{reduced} if and only if the
following hold: \begin{compactenum}
  %
\item\label{it1:reduced-td} for each $\arel \in \signature$ and each $\tuple{u_1, \ldots,
  u_{\arityof{\arel}}} \in \struc(\arel)$ there exists a leaf $n \in
  \tnodes$ such that $\set{u_1, \ldots, u_{\arityof{\arel}}} \subseteq
  \alabel(n)$, called the \emph{witness} of $\tuple{u_1, \ldots,
    u_{\arityof{\arel}}} \in \struc(\arel)$,
  %
\item\label{it2:reduced-td} every leaf witnesses exactly one tuple $\tuple{u_1, \ldots,
  u_{\arityof{\arel}}} \in \struc(\arel)$,
  %
\item\label{it3:reduced-td} $\tree$ is a binary tree i.e., a tree where each node has at
  most two children,
  %
\item\label{it4:reduced-td} if $n \in \tnodes$ has two children $m_1,m_2 \in \tnodes$
  then $\alabel(n) = \alabel(m_1) = \alabel(m_2)$,
  %
\item\label{it5:reduced-td} if $n \in \tnodes$ has one child $m \in \tnodes$ then either
  $\alabel(n) = \alabel(m)$ and $m$ witnesses a tuple $\tuple{u_1,
  \ldots, u_{\arityof{\arel}}} \in \struc(\arel)$, or
  $\cardof{\alabel(n) \setminus \alabel(m)} = \cardof{\alabel(m)
  \setminus \alabel(n)} = 1$,
  %
\item\label{it6:reduced-td} $\cardof{\alabel(n)} = k+1$, for all $n \in \tnodes$.
\end{compactenum}
\end{definition}
Considering only reduced tree decompositions is without loss of generality:

\begin{propositionE}\label{prop:reduced-tree-decompositions}
If a structure $\struc$ has a tree decomposition of width $k$, then it
also has a reduced tree decomposition of width $k$.
\end{propositionE}
\begin{proofE}
  The properties (\ref{it1:reduced-td}-\ref{it6:reduced-td}) can
  be proven directly from Definition~\ref{def:treewidth}. The main
  tool is the introduction of intermediate nodes into the tree
  decomposition. We list some of the cases. For
  (\ref{it1:reduced-td}), if a node witnesses more than one tuple,
  then we introduce an intermediate node between itself and its parent
  that is labeled by the same set of vertices. The intermediate node
  then becomes the witness for the this tuple. This process can be
  iterated until every node witnesses at most one tuple.  For
  (\ref{it3:reduced-td}), if a node $n_0$ has children
  $m_0,\cdots,m_l$ we can introduce new nodes $n_1,\ldots,n_{l-1}$
  with $\alabel(m_0) = \alabel(m_i)$, and create a new tree
  decomposition which agrees with the old tree decomposition except
  that we remove the edges from $n_0$ to the children $m_0,\cdots,m_l$
  and add edges from $n_i$ to $m_i$ and $n_{i+1}$ for all $i<l-1$ and
  edges from $n_{l-1}$ to $m_{l-1}$ and $m_l$.  For
  (\ref{it6:reduced-td}), note that we always consider structures over
  some infinite universe.  Hence, we can always extend the labels of
  the tree-decomposition with some fresh vertices from the
  universe. \qed
\end{proofE}
We make use of an additional unary relation symbol $\domsymb$, assumed
not to be part of $\signature$ i.e., the rules of the SID are written
using the signature $\signature \cup \set{\domsymb}$. The generic SID
$\asid_{\mathit{gen}}$ consists of the following rules, with the only
predicate symbol $\apred$ of arity $k+1$:
\begin{align}
  \apred(x_1, \ldots, x_{k+1}) \leftarrow & \apred(x_1, \ldots, x_{k+1}) * \apred(x_1, \ldots, x_{k+1}) *
  \Asterisk_{\!\!i, j \in \interv{1}{k+1}} x_i \!\neq\! x_j  \label{rule:gen-comp} \\
  \apred(x_1, \ldots, x_{k+1}) \leftarrow & \exists x_0 . \apred(x_1, \ldots,x_{k+1})[x_i/x_0] *
  \domsymb(x_0) * \Asterisk_{\!\!i, j \in \interv{0}{k+1}} x_i \!\neq\! x_j \label{rule:gen-exists} \\
  & \quad \quad \text{ for all } 1 \le i \le k+1 \nonumber \\
  \apred(x_1, \ldots, x_{k+1}) \leftarrow & \arel(y_1,\ldots,y_{\arityof{\arel}}) *
  \Asterisk_{\!\!i, j \in \interv{1}{k+1}} x_i \!\neq\! x_j \label{rule:gen-rel} \\
  & \quad \quad \text{ for any choice of } y_1,\ldots,y_{\arityof{\arel}} \text{  among } x_1, \ldots, x_{k+1} \nonumber
\end{align}
%
The following two lemmas prove that $\asid_{\mathit{gen}}$ indeed defines all
structures of treewidth at most $k$, over the signature $\signature$.

\begin{lemmaE}\label{lem:tree-decomposotion-implies-sid}
Let $\struc$ be a structure with $\twof{\struc} \le k$ witnessed by
some reduced tree decomposition $\tree=(\tnodes,\tedges,r,\alabel)$,
such that $\alabel(r)=\{\vertex_1,\ldots,\vertex_{k+1}\}$ and let
$\store$ be a store with $\store(x_i) = \vertex_i$. Then we have
$(\struc^\tree,\store) \models_{\asid_{\mathit{gen}}} \apred(x_1,
\ldots, x_{k+1})$, where $\struc^\tree$ is the structure $\struc$
extended by the unary relation $\domsymb$, such that
$\struc^\tree(\domsymb) = \bigcup_{n \in \tnodes}
\alabel(n) \setminus \{\vertex_1,\ldots,\vertex_{k+1}\}$.
\end{lemmaE}
\begin{proofE}
  The proof goes by induction on the structure of $\tree$.  The claim
  clearly holds for the base case, where $\tree$ consists of a single
  leaf, by rule (\ref{rule:gen-rel}). We assume the root of $\tree$
  has two children.  The subtrees $\tree_1$ and $\tree_2$ rooted in
  the two children induce substructures $\struc_1$ and $\struc_1$ of
  $\struc$, where $\tuple{u_1, \ldots,
  u_{\arityof{\arel}}} \in \struc_i(\arel)$ iff $\tuple{u_1, \ldots,
  u_{\arityof{\arel}}}$ is witnessed by some leaf of $\tree_i$, for $i
  = 1,2$. Because $\tree$ is a reduced tree decomposition, there is at
  most one leaf that witnesses a tuple $\tuple{u_1, \ldots,
  u_{\arityof{\arel}}} \in \struc_i(\arel)$.  Hence, we have $\struc
  = \struc_1 \comp \struc_2$. Because the only elements that can
  appear as labels in both $\tree_1$ and $\tree_2$ are
  $\{\vertex_1,\ldots,\vertex_{k+1}\}$, we also get that $\struc^\tree
  = \struc_1^{\tree_1} \comp \struc_2^{\tree_2}$. From the inductive
  hypothesis we obtain
  $(\struc_i^{\tree_i},\store) \models_{\asid_{\mathit{gen}}} \apred(x_1, \ldots,
  x_{k+1})$, for $i = 1,2$.  Hence
  $(\struc_1^{\tree_1} \comp \struc_2^{\tree_2},\store) \models_{\asid_\mathit{gen}} \apred(x_1, \ldots,
  x_{k+1}) * \apred(x_1, \ldots, x_{k+1})$, thus
  $(\struc,\store) \models_{\asid_{\mathit{gen}}} \apred(x_1, \ldots,
  x_{k+1})$, by rule (\ref{rule:gen-comp}). We now assume that the
  root of $\tree$ has a single child which is not a leaf and consider
  the subtree $\tree'$ rooted at this child. Then, there is an element
  $\vertex$ with $\vertex \neq \vertex_i$, for all $1 \le i \le k+1$,
  such that the root of $\tree'$ is labelled by
  $\{\vertex_1,\ldots,\vertex_{i-1},\vertex,\vertex_{i+1},\ldots,\vertex_{k+1}\}$.
  By the inductive hypothesis, we obtain
  $(\struc^{\tree'},\store[x_i \leftarrow \vertex]) \models_{\asid_{\mathit{gen}}} \apred(x_1, \ldots,
  x_{k+1})$.  We recognize that $\struc^{\tree'}$ agrees with
  $\struc^\tree$ except that $\vertex \in \struc^\tree(\domsymb)$.
  Hence, $(\struc^\tree,\store) \models_{\asid_{\mathit{gen}}} \exists
  x_0 ~.~ \apred(x_1,\ldots,x_{k+1})[x_i / x_0] * \domsymb(x_0)
  * \Asterisk_{0 \le i < j \le k+1} \ x_i \neq x_j$, thus
  $(\struc^\tree,\store) \models_{\asid_{\mathit{gen}}} \apred(x_1,\ldots,x_{k+1})$,
  by rule (\ref{rule:gen-exists}). \qed
\end{proofE}

\begin{lemmaE}
\label{lem:sid-implies-tree-decomposition}
Let $(\struc,\store)$ be a structure-store pair such that
$(\struc,\store) \models_{\asid_{\mathit{gen}}}
\apred(x_1,\ldots,x_{k+1})$ and $\store(x_i) \not\in \struc(\domsymb)$
for all $1 \le i \le k+1$. Then, there exists a reduced tree
decomposition $\tree = (\tnodes,\tedges,r,\alabel)$ of $\struc$, such
that $\twof{\tree}=k$,
$\alabel(r)=\set{\store(x_1),\ldots,\store(x_{k+1})}$ and $\alabel(n)
\subseteq \struc(\domsymb) \cup
\{\store(x_1),\ldots,\store(x_{k+1})\}$, for all $n \in \tnodes$.
\end{lemmaE}
\begin{proofE}
  We prove the claim by induction on the number of rule
  applications. The claim clearly holds for the base case. We now
  consider the rule (\ref{rule:gen-comp}) i.e., we assume that
  $(\struc,\store) \models_{\asid_{\mathit{gen}}} \apred(x_1,\ldots,x_{k+1})
  * \apred(x_1,\ldots,x_{k+1}) * \Asterisk_{1 \le i < j \le k+1} \
  x_i \neq x_j$. Then, there are structures $\struc_1$ and $\struc_2$
  with
  $(\struc_i,\store) \models_{\asid_{\mathit{gen}}} \apred(x_1,\ldots,x_{k+1})$,
  for $i = 1,2$ and $\struc_1 \comp \struc_2 = \struc$. We note that
  the latter implies that $\struc_1(\domsymb)$ and
  $\struc_2(\domsymb)$ are disjoint (*). We now apply the inductive
  hypothesis and obtain reduced tree decompositions $\tree_i$ for
  $\struc_i$ whose respective root is labelled by
  $\{\store(x_1),\ldots,\store(x_{k+1})\}$ and
  $\alabel(n) \subseteq \struc(\domsymb) \cup \{\store(x_1),\ldots,\store(x_{k+1})\}$,
  for all nodes $n$ of $\tree_i$ and all $i = 1,2$. We obtain a
  reduced tree decomposition for $\struc$ by composing $\tree_1$ and
  $\tree_2$ with a fresh root node labelled by
  $\{\store(x_1),\ldots,\store(x_{k+1})\}$. Note that $\tree$ is
  indeed a tree decomposition because by (*) the only elements that
  may appear in labels of both $\tree_1$ and $\tree_2$ must belong to
  $\{\store(x_1),\ldots,\store(x_{k+1})\}$. Clearly, we have
  $\alabel(n) \subseteq \struc_1(\domsymb) \cup \struc_2(\domsymb) \cup \{\store(x_1),\ldots,\store(x_{k+1})\}
  = \struc(\domsymb) \cup \{\store(x_1),\ldots,\store(x_{k+1})\}$, for
  all nodes $n$ of the resulting tree decomposition $\tree$. We now
  consider the rule (\ref{rule:gen-exists}) i.e., we assume that
  $(\struc,\store) \models_{\asid_{\mathit{gen}}} \exists x_0
  ~.~ \apred(x_1, \ldots,x_{k+1})[x_i/x_0] * \domsymb(x_0)
  * \Asterisk_{0 \le i < j \le k+1} \ x_i \neq x_j$.  Then, there is
  an element $\vertex \not\in \set{\vertex_1, \ldots, \vertex_{k+1}}$,
  such that
  $(\struc',\store[x_i \leftarrow \vertex]) \models_{\asid_{\mathit{gen}}} \apred(x_1, \ldots,x_{k+1})$,
  where the structure $\struc'$ agrees with $\struc$, except that
  $\struc(\domsymb) = \struc'(\domsymb) \setminus \set{\vertex}$.  We
  now apply the inductive hypothesis and obtain a reduced tree
  decomposition $\tree'$ for $\struc'$ whose root is labelled by
  $(\{\store(x_1),\ldots,\store(x_{k+1})\} \setminus \{\store(x_i)\}) \cup \{\vertex\}$
  and $\alabel(n) \subseteq
  ((\struc'(\domsymb) \cup \{\store(x_1),\ldots,\store(x_{k+1})\}) \setminus \{\store(x_i)\}) \cup \{\vertex\}$,
  for all nodes $n$ of $\tree'$ (\#).  We can now obtain a reduced
  tree decomposition $\tree$ for $\struc$ by composing $\tree'$ with
  an additional root labelled by
  $\{\store(x_1),\ldots,\store(x_{k+1})\}$.  Note that $\tree$ is
  indeed a tree decomposition because $\store(x_i) \not\in \alabel(n)$
  for every node $n$ of $\tree'$, because of (\#),
  $\vertex \neq \store(x_i)$ and the assumption that
  $\store(x_i) \not\in \struc(\domsymb)$.  We have
  $\alabel(n) \subseteq \struc'(\domsymb) \cup \{\store(x_1),\ldots,\store(x_{k+1})\} \cup \{\vertex\}
  = \struc(\domsymb) \cup \{\store(x_1),\ldots,\store(x_{k+1})\}$ for
  all nodes $n$ of the resulting tree decomposition $\tree$. \qed
\end{proofE}

We now want to track the satisfaction of all \mso\ formul{\ae} up to
quantifier-rank $\Rank$ over some signature $\signature$, in the
structures defined by the generic SID $\asid_{\mathit{gen}}$. To this
end, we consider the set $\types = \{ \thof^\Rank(\struc) \mid
\text{some } \signature\text{-structure } \struc\}$, where
$\thof^\Rank(\struc)$ denotes the set of all \mso\ sentences $\phi$ of
quantifier-rank at most $\Rank$, such that $\struc \Models \phi$. As
there are only finitely many logically equivalent sentences of
quantifier-rank at most $\Rank$, each $\thof^\Rank(\struc)$ can be
finitely represented e.g., by the Hintikka formul{\ae} describing
$\Rank$-round Ehrenfeucht–Fra\"iss\'e games
\cite{DBLP:books/daglib/0082516}. 
For such a finite representation of $\thof^\Rank(\struc)$ and some
sentence $\phi$ of quantifier-rank at most $\Rank$, it is known to be
decidable whether $\phi \in \thof^\Rank(\struc)$.

\begin{definition}\label{def:smooth}
An operation $\operation(\struc_1,\ldots,\struc_n)$ on structures is
called \emph{smooth} if and only if
$\thof^\Rank(\operation(\struc_1,\ldots,\struc_n))$ uniquely depends
on $\thof^\Rank(\struc_1),\ldots,\thof^\Rank(\struc_k)$. The operation
$\operation$ is called \emph{effectively smooth} if and only if there
is an effective method $\method_\operation$ for computing the finite
representation of $\thof^\Rank(\operation(\struc_1,...,\struc_n))$
from the finite representations of
$\thof^\Rank(\struc_1),...,\thof^\Rank(\struc_k)$.
\end{definition}

The \emph{fuse} operation $\fuse_U(\struc)$ on a unary relation symbol
$U \in \signature$, for a structure $\struc$ over a signature
$\signature$, is defined as the structure where all elements from the
interpretation of $U$ are contracted into a single element. Formally,
$\struc' = \fuse_U(\struc)$ is defined as $\struc$ if there is no
$\vertex \in \struc(U)$ or $\struc'$ is obtained from $\struc$ by
fixing some $\vertex \in \struc(U)$ and replacing for every relation
$\arel$ and every tuple $\tuple{\vertex_1, \ldots,
  \vertex_{\arityof{\arel}}} \in \struc(\arel)$ every $\vertex_i$ by
$\vertex$ in case $\vertex_i \in \struc(U)$.

A \emph{quantifier-free translation scheme}\footnote{We only consider
here very restricted translation schemes, where the source and target
structures are over the same signature and the structures have the
same domain; see~\cite{journals/apal/Makowsky04} for a general
definition of translation schemes.} over some signature $\signature$
is defined by a quantifier-free formula
$\phi_\arel(x_1,\ldots,x_{\arityof{\arel}})$, for every relation
symbol $\arel \in \signature$ (we require the formulae $\phi_\arel$ to
be also over signature $\signature$). Given a structure $\struc$ a
quantifier-free translation scheme defines a structure $\struc'$,
where $\tuple{\vertex_1, \ldots, \vertex_{\arityof{\arel}}} \in
\struc'(\arel) \iff \struc \models
\phi_\arel(\vertex_1,\ldots,\vertex_{\arityof{\arel}})$.

We rely on the following operations being effectively smooth
(see~\cite{journals/apal/Makowsky04}): \begin{compactitem}
  %
\item the \emph{composition} $\comp$ of two structures (see
  Definition~\ref{def:composition}); this relies on the fact that the
  union of standard structures defined on disjoint domains is
  effectively smooth and that we apply composition only between
  structures defined over the same universe $\universe$, that have
  disjoint interpretations of the $\domsymb$ relation, intended to
  simulate the domain of a structure, in the standard sense (see
  Remark \ref{rem:structures}),
  %
\item the \emph{fuse operation} ($\fuse_U$) is effectively smooth for
  structures over signatures that only consist of unary and binary
  relation symbols,
  %
\item \emph{quantifier-free translation schemes}.
\end{compactitem}

We now describe a refinement of the generic SID $\asid_{\mathit{gen}}$
intended to define all models of a given \mso\ formula, that have
treewidth at most $k$. We fix some signature $\signature$, consisting
of relation symbols of arity one or two, such that $\domsymb \not\in
\signature$.  While the predicates of the SID have free variables
$x_1,\ldots,x_{k+1}$, we encode the free variables by unary special
relations not from the considered signature i.e., $U_1,\ldots,U_{k+1}
\not\in \signature$.  For a structure $\struc$ over signature
$\signature$ and a store $\store$ with $\domain(\store) =
\{x_1,...,x_{k+1}\}$, we denote by $\encode(\struc,\store)$ the
structure over the extended signature $\signature \cup
\{U_1,...,U_{k+1} \}$ such that the unary relation $U_i$ is
interpreted as the singleton $\set{\store(x_i)}$, for all
$i \in \interv{1}{k+1}$. The refined SID $\asid_{\mathit{ref}}$ is
obtained as the product of the generic SID $\asid_{\mathit{gen}}$ and
the types $\types$ over $\signature \cup
\{U_1,\ldots,U_{k+1} \}$, for some fixed quantifier-rank $\Rank$,
using a set of predicates $\apred_\tau$, for $\tau \in \types$, consisting of the rules:
\vspace*{-.5\baselineskip}
\begin{align}
  \apred_\tau(x_1, \ldots, x_{k+1}) \leftarrow & \apred_{\omega_1}(x_1, \ldots, x_{k+1}) *
  \apred_{\omega_2}(x_1, \ldots, x_{k+1}) * \Asterisk_{\!\!i,j \in \interv{1}{k+1}} x_i \!\neq\! x_j  \label{rule:ref-comp} \\
  % & \quad \quad \text{with } \tau,\omega_1,\omega_2 \in \types \nonumber\\
  & \quad \quad  \text{where } \tau = \method_{\fuse_{U_1}} \circ  \cdots \circ \method_{\fuse_{U_{k+1}}} \circ \method_\comp(\omega_1,\omega_2) \nonumber
\end{align}
\begin{align}
  \apred_\tau(x_1, \ldots, x_{k+1}) \leftarrow & \exists x_0 ~.~ \apred_\omega(x_1, \ldots,x_{k+1})[x_\ell/x_0] * \domsymb(x_0) *
  \Asterisk_{i,j \in \interv{0}{k+1}} x_i \!\neq\! x_j \label{rule:ref-exists} \\
  & \quad \quad \text{where } \tau = \method_\comp(m_{\rlandf_{U_\ell}}(\omega),\thof(\struc_\ell)) \text{ and } \struc_\ell \text{ is} \nonumber \\
  & \quad \quad \text{the structure with a single element labeled by } U_\ell, \nonumber \\
  & \quad \quad \text{for all } \ell \in \interv{1}{k+1}, \nonumber \\
  \apred_\tau(x_1, \ldots, x_{k+1}) \leftarrow & \arel(y_1,\ldots,y_{\arityof{\arel}}) * \Asterisk_{i, j \in \interv{1}{k+1}} x_i \!\neq\! x_j \label{rule:ref-rel} \\
    & \quad \quad \text{for any choice of } y_1,\ldots,y_{\arityof{\arel}} \text{  among the } x_1, \ldots, x_{k+1}, \nonumber \\[-1mm]
    & \quad \quad \text{where } \tau = \thof(\struc) \text{ for some structure } \struc \text{, where } \struc(U_\ell)=\set{u_\ell} \nonumber \\[-1mm]
    & \quad \quad \text{for some } u_1, \ldots, u_{k+1} \text{ and } \struc(\arel) = \set{\tuple{v_1, \ldots, v_{\arityof{\arel}}}} \nonumber \\[-1mm]
    % & \quad \quad \text{pairwise different elements } \vertex_\ell \text{ are labelled by } U_\ell,~ \ell\in\interv{1}{k+1}\nonumber \\[-1mm]
    % & \quad \quad \text{and } \arel \text{ is interpreted by the singleton } \set{\tuple{v_1,\ldots,v_{\arityof{\arel}}}}, \nonumber \\[-1mm]
    & \quad \quad \text{with } v_1,...,v_{\arityof{\arel}} \text{ chosen among } \vertex_1,\ldots,\vertex_{k+1} \nonumber \\[-1mm]
    & \quad \quad \text{as } y_1,\ldots,y_{\arityof{\arel}} \text{ are chosen among } x_1, \ldots, x_{k+1} \nonumber
\end{align}
In the above rules, $\rlandf_{U_\ell}$ is the translation scheme
defined by the identity, for all relations $\arel$ apart from $U_\ell$
and $\domsymb$ i.e., $\phi_{\arel(x_1,\ldots,x_{\arityof{\arel}})} =
\arel(x_1,\ldots,x_{\arityof{\arel}})$, $\phi_{U_\ell}(x) :=
\mathit{false}$ and $\phi_\domsymb(x) := \domsymb(x) \vee U_\ell(x)$.
We prove the properties of $\asid_{\mathit{ref}}$:

\begin{lemmaE}\label{lem:refined-SID-is-sound}
Let $(\struc,\store)$ be a structure-store pair such that
$(\struc,\store) \models_{\asid_{\mathit{ref}}} \apred_\tau(x_1,
\ldots, x_{k+1})$ and $\store(x_i) \not\in \struc(\domsymb)$, for all
$i \in \interv{1}{k+1}$. Then, we have
$\thof(\encode(\struc^{-\domsymb},\store)) = \tau$, where
$\struc^{-\domsymb}$ is the structure obtained from $\struc$ by
ignoring the interpretation of $\domsymb$.
\end{lemmaE}
\begin{proofE}
  We prove the claim by induction on the number of rule applications.
  Clearly the claim holds for the base case, by rule
  (\ref{rule:ref-rel}). We now consider the rule (\ref{rule:ref-comp})
  i.e., we have
  $(\struc,\store) \models_{\asid_{\mathit{ref}}} \apred_{\omega_1}(x_1, \ldots,
  x_{k+1}) * \apred_{\omega_2}(x_1, \ldots, x_{k+1})
  * \Asterisk_{i,j \in \interv{1}{k+1}} \ x_i \neq x_j$. Then, there
  are structures $\struc_1$ and $\struc_2$ with
  $(\struc_i, \store) \models_{\asid_{\mathit{ref}}} \apred_{\omega_i}(x_1, \ldots,
  x_{k+1})$, for $i = 1,2$ and $\struc_1 \comp \struc_2 = \struc$.  We
  note that the latter implies that
  $\struc_1(\domsymb)\cap\struc_2(\domsymb)=\emptyset$ (*). By
  Lemma~\ref{lem:sid-implies-tree-decomposition}, we have that
  $\struc_i$ has a tree decomposition
  $\tree_i=(\tnodes_i,\tedges_i,r_i,\alabel_i)$, with
  $\alabel_i(n) \subseteq \struc(\domsymb) \cup \{\store(x_1),\ldots,\store(x_{k+1})\}$,
  for all $n\in\tnodes_i$ and $i=1,2$ (\#).  By the inductive
  hypothesis, we have that
  $\thof(\encode(\struc_i^{-\domsymb},\store)) = \omega_i$, for
  $i=1,2$.  We now note that while $\struc_1$ and $\struc_2$ are
  disjoint, $\encode(\struc_1^{-\domsymb},\store)$ and
  $\encode(\struc_2^{-\domsymb},\store))$ will not be disjoint (as
  they overlap for the unary relations $U_i$).  Hence, we will
  consider some structure $\struc_2'$ that agrees with $\struc_2$
  apart from the elements in the image of $\store$: We first choose
  some store $\store'$ with
  $\store'(x_i) \not\in \struc(\domsymb_1) \cup \struc(\domsymb_2) \cup \{\store(x_1),\ldots,\store(x_{k+1})\}$.
  We then choose a bijection $h$ from
  $\struc_2(\domsymb) \cup \{\store(x_1),\ldots,\store(x_{k+1})\}$ to
  $\struc_2(\domsymb) \cup \{\store'(x_1),\ldots,\store'(x_{k+1})\}$,
  which is the identity on
  $\struc(\domsymb) \setminus \{\store(x_1),\ldots,\store(x_{k+1})\}$.
  Let $\struc_2'$ be the isomorphic structure induced by $h$ on
  $\struc_2$.  We now observe that
  $\encode(\struc_1^{-\domsymb},\store)$ and
  $\encode(\struc_2'^{-\domsymb},\store'))$ are disjoint, by (*) and
  (\#).  We also note that $\encode(\struc_2'^{-\domsymb},\store'))
  = \encode(\struc_2^{-\domsymb},\store)) = \omega_2$, by
  Prop. \ref{prop:so-iso}. We finally note that
  $\encode(\struc^{-\domsymb},\store)$ can be obtained from
  $\encode(\struc_1^{-\domsymb},\store)$ and
  $\encode(\struc_2'^{-\domsymb},\store'))$ by the disjoint union and
  fuse operations, i.e., $\encode(\struc^{-\domsymb},\store)
  = \fuse_{U_1} \circ \cdots \circ \fuse_{U_{k+1}} \circ
  ( \encode(\struc_1^{-\domsymb},\store) \comp \encode(\struc_2^{-\domsymb},\store))$. By
  the smoothness of $\fuse$ and $\comp$ we obtain:
  \[\begin{array}{l}
  \thof(\encode(\struc^{-\domsymb},\store)) = \\
  \method_{\fuse_{U_1}} \circ \cdots \circ \method_{\fuse_{U_{k+1}}} \circ
  \method_\comp(\thof(\encode(\struc_1^{-\domsymb},\store)),\thof(\encode(\struc_2^{-\domsymb},\store))) = \\
  \method_{\fuse_{U_1}} \circ \cdots \circ \method_{\fuse_{U_{k+1}}} \circ \method_\comp(\omega_1,\omega_2) = \tau
  \end{array}\] We now consider the rule (\ref{rule:ref-exists}) i.e., we have
  $(\struc, \store) \models_{\asid_{\mathit{ref}}} \exists x_0
  ~.~ \apred_\tau(x_1, \ldots,x_{k+1})[x_i/x_0] * \domsymb(x_0)
  * \Asterisk_{i,j \in \interv{1}{k+1}}\ x_i \neq x_j$. Then, there is
  an element $\vertex$ with $\vertex \neq \vertex_i$, for all $1 \le
  i \le k+1$ such that
  $(\struc',\store[x_i \leftarrow \vertex]) \models_{\asid_{\mathit{ref}}} \apred(x_1, \ldots,x_{k+1})$,
  where the structure $\struc'$ agrees with $\struc$, except for
  $\struc(\domsymb) = \struc'(\domsymb) \setminus \set{\vertex}$. By
  the Lemma \ref{lem:sid-implies-tree-decomposition}, there is a tree
  decomposition $\tree'=(\tnodes',\tedges',r',\alabel')$ for $\struc'$
  with
  $\alabel'(n) \subseteq \struc(\domsymb) \cup \{\store(x_1),\ldots,\store(x_{k+1})\}$
  for all $n\in\tnodes'$. By the inductive hypothesis, we have that
  $\thof(\encode(\struc'^{-\domsymb},\store[x_i \leftarrow \vertex]))
  = \omega$. We now observe that $\encode(\struc^{-\domsymb},\store)
  = \rlandf_{U_i}(\encode(\struc'^{-\domsymb},\store[x_i \leftarrow \vertex])) \comp \struc_i$,
  where $\struc_i$ is the structure for which only the element
  $\store(x_i)$ is labelled by $U_i$. By the smoothness of $\rlandf$
  and $\comp$, we obtain:
  \[\begin{array}{l}
  \thof(\encode(\struc^{-\domsymb},\store)) = \\
  \method_\comp(m_{\rlandf_{U_i}}(\thof(\encode(\struc'^{-\domsymb},\store[x_i \leftarrow \vertex]))),\thof(\struc_i)) = \\
  \method_\comp(m_{\rlandf_{U_i}}(\omega),\thof(\struc_i)) = \tau \hspace*{.5\textwidth}\text{\qed}
  \end{array}\]
\end{proofE}

\begin{lemmaE}\label{lem:refined-SID-is-complete}
Let $(\struc,\store)$ be a structure-store pair, such that
$\thof(\encode(\struc,\store)) = \tau$, $\store(x_i) \neq \store(x_j)$
for all $i \neq j$ and $\twof{\struc} \le k$, witnessed by some
reduced tree decomposition $\tree=(\tnodes,\tedges,r,\alabel)$.  Then,
we have $(\struc^\tree,\store) \models_{\asid_{\mathit{ref}}}
\apred_\tau(x_1, \ldots, x_{k+1})$.
\end{lemmaE}
\begin{proofE}
  The proof proceeds by induction on the structure of $\tree$.
  Clearly the claim holds for the base case, by rule
  (\ref{rule:ref-rel}). We assume that the root of $\tree$ has two
  children. The subtrees $\tree_1$ and $\tree_2$ rooted in the two
  children induce substructures $\struc_1$ and $\struc_1$ of $\struc$,
  where $\tuple{u_1, \ldots, u_{\arityof{\arel}}} \in \struc_i(\arel)$
  iff $\tuple{u_1, \ldots, u_{\arityof{\arel}}}$ is witnessed by some
  leaf of the respective subtree.  Because $\tree$ is a reduced tree
  decomposition, there is at most one leaf that witnesses a tuple
  $\tuple{u_1, \ldots,
  u_{\arityof{\arel}}} \in \struc_i(\arel)$. Hence, we have $\struc
  = \struc_1 \comp \struc_2$.  Because the only elements that can
  appear as labels in $\tree_1$ and $\tree_2$ are
  $\{\store(x_1),\ldots,\store(x_{k+1})\}$, we also get that
  $\struc^\tree = \struc_1^{\tree_1} \comp \struc_2^{\tree_2}$.  Let
  $\omega_i = \thof(\encode(\struc_i,\store))$. From the inductive
  hypothesis, we obtain
  $(\struc_i^{\tree_i},\store) \models_{\asid_{\mathit{ref}}} \apred_{\omega_i}(x_1, \ldots,
  x_{k+1})$, for $i=1,2$. Let $\tau
  = \method_{\fuse_{U_1}} \circ \cdots \circ \method_{\fuse_{U_{k+1}}} \circ \method_\comp(\omega_1,\omega_2)$. As
  in the proof of Lemma~\ref{lem:refined-SID-is-complete}, we can now
  show that $\thof(\encode(\struc,\store)) = \tau$.  Hence, we now get
  that
  $(\struc_1^{\tree_1} \comp \struc_2^{\tree_2},\store) \models_{\asid_{\mathit{ref}}} \apred_{\omega_1}(x_1, \ldots,
  x_{k+1}) * \apred_{\omega_2}(x_1, \ldots, x_{k+1})$ i.e., that
  $(\struc^\tree,\store) \models_{\asid_{\mathit{ref}}} \apred_\tau(x_1, \ldots,
  x_{k+1})$ by rule (\ref{rule:ref-comp}). We now assume that the root
  of $\tree$ has a single child which is not a leaf.  We consider the
  subtree $\tree'$ rooted at this child.  Then, there is an element
  $\vertex$ with $\vertex \neq \store(x_i)$, for all $1 \le i \le k+1$
  such that the root of $\tree'$ is labeled by
  $\{\store(x_1),\ldots,\store(x_{i-1}),\vertex,\store(x_{i+1}),\ldots,\store(x_{k+1})\}$.
  Let $\omega
  = \thof(\encode(\struc,\store[x_i \leftarrow \vertex]))$.  By the
  inductive hypothesis, we obtain that
  $(\struc^{\tree'},\store[x_i \leftarrow \vertex]) \models_{\asid_{\mathit{ref}}} \apred_\omega(x_1, \ldots,
  x_{k+1})$.  Let $\tau
  = \method_\comp(m_{\rlandf_{X_i}}(\omega),\thof(\struc'))$, where
  $\struc'$ is the structure for which the single element
  $\store(x_i)$ is labeled by $U_i$. As in the proof of
  Lemma~\ref{lem:refined-SID-is-complete}, we can now show that
  $\thof(\encode(\struc,\store)) = \tau$. We now recognize that
  $\struc^{\tree'}$ agrees with $\struc^\tree$ except that
  $\struc^{\tree}(\domsymb)
  = \struc^{\tree'}(\domsymb) \cup \set{\vertex}$. Hence, we get that
  $(\struc^\tree,\store) \models_{\asid_{\mathit{ref}}} \exists x_0
  ~.~ \apred_\tau(x_1, \ldots,x_{k+1})[x_i/x_0] * \domsymb(x_0)
  * \Asterisk_{i,j \in \interv{1}{k+1}} \ x_i \neq x_j$ i.e., that
  $(\struc^\tree,\store) \models_{\asid_{\mathit{ref}}} \apred_\tau(x_1, \ldots,
  x_{k+1})$ by rule (\ref{rule:ref-exists}). \qed
\end{proofE}

In order to define the models of an MSO sentence $\phi$ with
quantifier-free rank up to $\Rank$, we consider the rules
$\apred_\phi() \leftarrow \exists x_1 \ldots \exists x_{k+1} ~.~
\apred_\tau(x_1, \ldots, x_{k+1})$, for all $\tau \in \types$, such
that $\phi \in \tau$.

We believe that one can extend the approach presented above to
relations of higher arity by encoding such relations in terms of
binary relations (using that we are only interested in graphs of
bounded tree-width). We leave such details for future work.

As a final remark, by applying the translation of \slr\ to \sol\ from
\S\ref{sec:slr-so} to $\asid_{\mathit{gen}}$ and
$\asid_{\mathit{ref}}$ and taking the conjunction of the results, we
obtain an \sol\ formula that defines the models of an \slr\ formula of
treewidth at most $k$, allowing to infer that \slr\ $\subseteq^k$ \sol.

